DENOASR: Debiasing ASRs through Selective Denoising

Automatic Speech Recognition (ASR) systems have been examined and shown to exhibit biases toward particular groups of individuals, influenced by factors such as demographic traits, accents, and speech styles. Noise can disproportionately impact speakers with certain accents, dialects, or speaking styles, leading to biased error rates. In this work, we introduce a novel framework DENOASR, which is a selective denoising technique to reduce the disparity in the word error rates between the two gender groups, male and female. We find that a combination of two popular speech denoising techniques, viz. DEMUCS and LE, can be effectively used to mitigate ASR disparity without compromising their overall performance. Experiments using two state-of-the-art open-source ASRs - OpenAI WHISPER and NVIDIA NEMO - on multiple benchmark datasets, including TIE, VOX-POPULI, TEDLIUM, and FLEURS, show that there is a promising reduction in the average word error rate gap across the two gender groups. For a given dataset, the denoising is selectively applied on speech samples having speech intelligibility below a certain threshold, estimated using a small validation sample, thus ameliorating the need for large-scale human-written ground-truth transcripts. Our findings suggest that selective denoising can be an elegant approach to mitigate biases in present-day ASR systems.

==> References.tex <==
\begin{thebibliography}{00}



\bibitem[garnerin2019gender]{M. Garnerin, S. Rossato, and L. Besacier, ‘Gender representation in French broadcast corpora and its impact on ASR performance’, in Proceedings of the 1st international workshop on AI for smart TV content production, access and delivery, 2019, pp. 3–9.}


@article{hannun2021history,
  title={The history of speech recognition to the year 2030},
  author={Hannun, Awni},
  journal={arXiv preprint arXiv:2108.00084},
  year={2021}
}

@inproceedings{ngueajio2022hey,
  title={Hey ASR system! Why aren’t you more inclusive? Automatic speech recognition systems’ bias and proposed bias mitigation techniques. A literature review},
  author={Ngueajio, Mikel K and Washington, Gloria},
  booktitle={International Conference on Human-Computer Interaction},
  pages={421--440},
  year={2022},
  organization={Springer}
}

@article{koenecke2020racial,
  title={Racial disparities in automated speech recognition},
  author={Koenecke, Allison and Nam, Andrew and Lake, Emily and Nudell, Joe and Quartey, Minnie and Mengesha, Zion and Toups, Connor and Rickford, John R and Jurafsky, Dan and Goel, Sharad},
  journal={PNAS},
  year={2020},
}

@misc{alexa,
	author = {Amazon},
	title = {Alexa},
	howpublished = {\url{https://developer.amazon.com/en-US/alexa}},
	year = {2014},
	note = {Accessed: 2023-01-01}
}

@misc{Youtube_Live,
	author = {Google},
	title = {YouTube Automatic Captions},
	howpublished = {\url{https://ai.googleblog.com/2009/12/automatic-captioning-in-youtube.html?showComment=1263378133488}},
	year = {2009},
	note = {Accessed: 2023-01-01}
}

@misc{Cortana_Live,
	author = {Microsoft},
	title = {Cortana},
	howpublished = {\url{https://support.microsoft.com/en-us/topic/what-is-cortana-953e648d-5668-e017-1341-7f26f7d0f825}},
	year = {2014},
	note = {Accessed: 2023-01-01}
}

@misc{Zoom_Live,
	author = {Zoom Video Communications, Inc.},
	title = {Zoom Auto Generated Captions},
	howpublished = {\url{https://blog.zoom.us/zoom-auto-generated-captions/}},
	year = {2017},
	note = {Accessed: 2023-01-01}
}

@misc{Siri_Live,
	author = {Apple},
	title = {Siri},
	howpublished = {\url{https://support.apple.com/en-us/HT204389}},
	year = {2010},
	note = {Accessed: 2023-01-01}
}

@misc{Bing_Speech,
	author = {Microsoft},
	title = {Bing Speech},
	howpublished = {\url{https://azure.microsoft.com/en-us/products/ai-services/ai-speech}},
	year = {2015},
	note = {Accessed: 2023-01-01}
}



@article{baevski2020wav2vec,
  title={wav2vec 2.0: A framework for self-supervised learning of speech representations},
  author={Baevski, Alexei and Zhou, Yuhao and Mohamed, Abdelrahman and Auli, Michael},
  journal={NeurIPS},
  volume={33},
  pages={12449--12460},
  year={2020}
}

@article{radford2022robust,
  title={Robust speech recognition via large-scale weak supervision},
  author={Radford, Alec and Kim, Jong Wook and Xu, Tao and Brockman, Greg and McLeavey, Christine and Sutskever, Ilya},
  journal={arXiv preprint arXiv:2212.04356},
  year={2022}
}

@article{hannun2014deep,
  title={Deep speech: Scaling up end-to-end speech recognition},
  author={Hannun, Awni and Case, Carl and Casper, Jared and Catanzaro, Bryan and Diamos, Greg and Elsen, Erich and Prenger, Ryan and Satheesh, Sanjeev and Sengupta, Shubho and Coates, Adam and others},
  journal={arXiv preprint arXiv:1412.5567},
  year={2014}
}

@inproceedings{povey2011kaldi,
  title={The Kaldi speech recognition toolkit},
  author={Povey, Daniel and Ghoshal, Arnab and Boulianne, Gilles and Burget, Lukas and Glembek, Ondrej and Goel, Nagendra and Hannemann, Mirko and Motlicek, Petr and Qian, Yanmin and Schwarz, Petr and others},
  booktitle={IEEE 2011 workshop on automatic speech recognition and understanding},
  number={CONF},
  year={2011},
  organization={IEEE Signal Processing Society}
}

@inproceedings{tatman2017effects,
  title={Effects of Talker Dialect, Gender \& Race on Accuracy of Bing Speech and YouTube Automatic Captions.},
  author={Tatman, Rachael and Kasten, Conner},
  booktitle={Interspeech},
  pages={934--938},
  year={2017}
}

@inproceedings{tatman2017gender,
  title={Gender and dialect bias in YouTube’s automatic captions},
  author={Tatman, Rachael},
  booktitle={EthNLP},
  pages={53--59},
  year={2017}
}

@inproceedings{meyer2020artie,
  title={Artie bias corpus: An open dataset for detecting demographic bias in speech applications},
  author={Meyer, Josh and Rauchenstein, Lindy and Eisenberg, Joshua D and Howell, Nicholas},
  booktitle={LREC},
  pages={6462--6468},
  year={2020}
}

@article{rai2023deep,
  title={A Deep Dive into the Disparity of Word Error Rates Across Thousands of NPTEL MOOC Videos},
  author={Rai, Anand Kumar and Jaiswal, Siddharth D and Mukherjee, Animesh},
  journal={AAAI ICWSM. To Appear.},
  year={2024}
}

@inproceedings{liu2022towards,
  title={Towards measuring fairness in speech recognition: Casual conversations dataset transcriptions},
  author={Liu, Chunxi and Picheny, Michael and Sar{\i}, Leda and Chitkara, Pooja and Xiao, Alex and Zhang, Xiaohui and Chou, Mark and Alvarado, Andres and Hazirbas, Caner and Saraf, Yatharth},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6162--6166},
  year={2022},
  organization={IEEE}
}

@book{AAVE,
  title = {Phonological and Grammatical Features of African American Vernacular (AAVE)},
  author = {Rickford, J. R.},
  publisher = {Blackwell Publishers},
  year = {1999}
}

@article{wang2021voxpopuli,
  title={VoxPopuli: A large-scale multilingual speech corpus for representation learning, semi-supervised learning and interpretation},
  author={Wang, Changhan and Riviere, Morgane and Lee, Ann and Wu, Anne and Talnikar, Chaitanya and Haziza, Daniel and Williamson, Mary and Pino, Juan and Dupoux, Emmanuel},
  journal={arXiv preprint arXiv:2101.00390},
  year={2021}
}

@inproceedings{krishnan2009nptel,
  title={NPTEL: A programme for free online and open engineering and science education},
  author={Krishnan, Mangala Sunder},
  booktitle={T4E},
  pages={1--5},
  year={2009},
  organization={IEEE}
}

@inproceedings{vu2014improving,
  title={Improving ASR performance on non-native speech using multilingual and crosslingual information},
  author={Vu, Ngoc Thang and Wang, Yuanfan and Klose, Marten and Mihaylova, Zlatka and Schultz, Tanja},
  booktitle={Interspeech},
  year={2014}
}

@article{sullivan2022improving,
  title={Improving automatic speech recognition for non-native english with transfer learning and language model decoding},
  author={Sullivan, Peter and Shibano, Toshiko and Abdul-Mageed, Muhammad},
  journal={arXiv preprint arXiv:2202.05209},
  year={2022}
}
@inproceedings{panayotov2015librispeech,
  title={Librispeech: an asr corpus based on public domain audio books},
  author={Panayotov, Vassil and Chen, Guoguo and Povey, Daniel and Khudanpur, Sanjeev},
  booktitle={2015 IEEE international conference on acoustics, speech and signal processing (ICASSP)},
  pages={5206--5210},
  year={2015},
  organization={IEEE}
}

@inproceedings{zhangcomparing,
  title={Comparing data augmentation and training techniques to reduce bias against non-native accents in hybrid speech recognition systems},
  author={Zhang, Yixuan and Zhang, Yuanyuan and Patel, Tanvina and Scharenborg, Odette},
  booktitle={Proc. 1st Workshop on Speech for Social Good (S4SG)},
  pages={15--19}
}

@article{feng2021quantifying,
  title={Quantifying bias in automatic speech recognition},
  author={Feng, Siyuan and Kudina, Olya and Halpern, Bence Mark and Scharenborg, Odette},
  journal={arXiv preprint arXiv:2103.15122},
  year={2021}
}

@inproceedings{garnerin2021investigating,
  title={Investigating the impact of gender representation in ASR training data: A case study on librispeech},
  author={Garnerin, Mahault and Rossato, Solange and Besacier, Laurent},
  booktitle={3rd Workshop on Gender Bias in Natural Language Processing},
  pages={86--92},
  year={2021},
  organization={Association for Computational Linguistics}
}

@article{winata2020learning,
  title={Learning fast adaptation on cross-accented speech recognition},
  author={Winata, Genta Indra and Cahyawijaya, Samuel and Liu, Zihan and Lin, Zhaojiang and Madotto, Andrea and Xu, Peng and Fung, Pascale},
  journal={arXiv preprint arXiv:2003.01901},
  year={2020}
}

@inproceedings{sriranjani2015improved,
  title={Improved acoustic modeling for automatic dysarthric speech recognition},
  author={Sriranjani, R and Reddy, M Ramasubba and Umesh, Srinivasan},
  booktitle={2015 Twenty First National Conference on Communications (NCC)},
  pages={1--6},
  year={2015},
  organization={IEEE}
}

@article{saadany2022better,
  title={Better Transcription of UK Supreme Court Hearings},
  author={Saadany, Hadeel and Or{\u{a}}san, Constantin and Breslin, Catherine},
  journal={arXiv preprint arXiv:2211.17094},
  year={2022}
}

@article{dheram2022toward,
  title={Toward fairness in speech recognition: Discovery and mitigation of performance disparities},
  author={Dheram, Pranav and Ramakrishnan, Murugesan and Raju, Anirudh and Chen, I-Fan and King, Brian and Powell, Katherine and Saboowala, Melissa and Shetty, Karan and Stolcke, Andreas},
  journal={arXiv preprint arXiv:2207.11345},
  year={2022}
}

@article{li2014overview,
  title={An overview of noise-robust automatic speech recognition},
  author={Li, Jinyu and Deng, Li and Gong, Yifan and Haeb-Umbach, Reinhold},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={22},
  number={4},
  pages={745--777},
  year={2014},
  publisher={IEEE}
}

@inproceedings{chao2021tenet,
  title={TENET: A time-reversal enhancement network for noise-robust ASR},
  author={Chao, Fu-An and Jiang, Shao-Wei Fan and Yan, Bi-Cheng and Hung, Jeih-weih and Chen, Berlin},
  booktitle={2021 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
  pages={55--61},
  year={2021},
  organization={IEEE}
}

@article{yadava2022enhancements,
  title={Enhancements in Continuous Kannada ASR System by Background Noise Elimination},
  author={Yadava, G Thimmaraja and Nagaraja, BG and Jayanna, Haradagere Siddaramaiah},
  journal={Circuits, Systems, and Signal Processing},
  volume={41},
  number={7},
  pages={4041--4067},
  year={2022},
  publisher={Springer}
}

@article{sainburg2020finding,
  title={Finding, visualizing, and quantifying latent structure across diverse animal vocal repertoires},
  author={Sainburg, Tim and Thielk, Marvin and Gentner, Timothy Q},
  journal={PLoS computational biology},
  volume={16},
  number={10},
  pages={e1008228},
  year={2020},
  publisher={Public Library of Science}
}

@software{tim_sainburg_2019_3243139,
  author       = {Tim Sainburg},
  title        = {timsainb/noisereduce: v1.0},
  month        = jun,
  year         = 2019,
  publisher    = {Zenodo},
  version      = {db94fe2},
  doi          = {10.5281/zenodo.3243139},
  url          = {https://doi.org/10.5281/zenodo.3243139}
}

@article{loshchilov2017decoupled,
  title={Decoupled weight decay regularization},
  author={Loshchilov, Ilya and Hutter, Frank},
  journal={arXiv preprint arXiv:1711.05101},
  year={2017}
}

@article{karraz2021effect,
  title={Effect of adaptive line enhancement filters on noise cancellation in ECG signals},
  author={Karraz, George},
  journal={SJEE},
  volume={18},
  number={3},
  pages={291--302},
  year={2021}
}



@article{vipperla2010ageing,
  title={Ageing voices: The effect of changes in voice parameters on ASR performance},
  author={Vipperla, Ravichander and Renals, Steve and Frankel, Joe},
  journal={EURASIP Journal on Audio, Speech, and Music Processing},
  pages={1--10},
  year={2010},
  publisher={Springer}
}

@article{shahamiri2021speech,
  title={Speech vision: An end-to-end deep learning-based dysarthric automatic speech recognition system},
  author={Shahamiri, Seyed Reza},
  journal={IEEE Transactions on Neural Systems and Rehabilitation Engineering},
  volume={29},
  pages={852--861},
  year={2021},
  publisher={IEEE}
}

@article{dichristofano2022performance,
  title={Performance disparities between accents in automatic speech recognition},
  author={DiChristofano, Alex and Shuster, Henry and Chandra, Shefali and Patwari, Neal},
  journal={arXiv preprint arXiv:2208.01157},
  year={2022}
}

@article{tu2016relationship,
  title={The relationship between perceptual disturbances in dysarthric speech and automatic speech recognition performance},
  author={Tu, Ming and Wisler, Alan and Berisha, Visar and Liss, Julie M},
  journal={The Journal of the Acoustical Society of America},
  volume={140},
  number={5},
  pages={EL416--EL422},
  year={2016},
  publisher={AIP Publishing}
}

@inproceedings{narayanan2014joint,
  title={Joint noise adaptive training for robust automatic speech recognition},
  author={Narayanan, Arun and Wang, DeLiang},
  booktitle={2014 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={2504--2508},
  year={2014},
  organization={IEEE}
}


@article{sari2021counterfactually,
  title={Counterfactually fair automatic speech recognition},
  author={Sar{\i}, Leda and Hasegawa-Johnson, Mark and Yoo, Chang D},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={29},
  pages={3515--3525},
  year={2021},
  publisher={IEEE}
}

@article{yu2020speech,
  title={Speech enhancement based on denoising autoencoder with multi-branched encoders},
  author={Yu, Cheng and Zezario, Ryandhimas E and Wang, Syu-Siang and Sherman, Jonathan and Hsieh, Yi-Yen and Lu, Xugang and Wang, Hsin-Min and Tsao, Yu},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={28},
  pages={2756--2769},
  year={2020},
  publisher={IEEE}
}

@inproceedings{weninger2015speech,
  title={Speech enhancement with LSTM recurrent neural networks and its application to noise-robust ASR},
  author={Weninger, Felix and Erdogan, Hakan and Watanabe, Shinji and Vincent, Emmanuel and Le Roux, Jonathan and Hershey, John R and Schuller, Bj{\"o}rn},
  booktitle={Latent Variable Analysis and Signal Separation: 12th International Conference, LVA/ICA 2015, Liberec, Czech Republic, August 25-28, 2015, Proceedings 12},
  pages={91--99},
  year={2015},
  organization={Springer}
}

@inproceedings{zhu2023robust,
  title={Robust data2vec: Noise-robust speech representation learning for asr by combining regression and improved contrastive learning},
  author={Zhu, Qiu-Shi and Zhou, Long and Zhang, Jie and Liu, Shu-Jie and Hu, Yu-Chen and Dai, Li-Rong},
  booktitle={ICASSP 2023-2023 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={1--5},
  year={2023},
  organization={IEEE}
}

@article{vaseghi1996spectral,
  title={Spectral subtraction},
  author={Vaseghi, Saeed V and Vaseghi, Saeed V},
  journal={Advanced Signal Processing and Digital Noise Reduction},
  pages={242--260},
  year={1996},
  publisher={Springer}
}

@article{venkateswarlu2011improve,
  title={Improve Speech Enhancement Using Weiner Filtering},
  author={Venkateswarlu, S China and Prasad, K Satya and Reddy, A SubbaRami and others},
  journal={Global Journal of Computer Science and Technology},
  volume={11},
  number={7},
  year={2011}
}

@article{michelsanti2021overview,
  title={An overview of deep-learning-based audio-visual speech enhancement and separation},
  author={Michelsanti, Daniel and Tan, Zheng-Hua and Zhang, Shi-Xiong and Xu, Yong and Yu, Meng and Yu, Dong and Jensen, Jesper},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={29},
  pages={1368--1396},
  year={2021},
  publisher={IEEE}
}

@article{burwen,
    author = {Burwen, Richard S.},
    title = "Design of a Noise Eliminator System",
    journal = {Journal of the Audio Engineering Society},
    year = 1971,
volume= 19,
issue=11,
pages={906–-911}
}

@book{records,
    author = {Hodgson, Jay},
    title = {Understanding Records},
    publisher = {Continuum Publishing Corporation},
    year = 2020,
isbn={978-1-4411-5607-5}
}

@book{hodgson2010understanding,
  author = {Hodgson, Jay},
  title = {Understanding Records: A Field Guide to Recording Practice},
  publisher = {Continuum International Publishing Group},
  year = {2010},
  pages = {272},
}

@article{yuliani2021speech,
  title={Speech enhancement using deep learning methods: A review},
  author={Yuliani, Asri Rizki and Amri, M Faizal and Suryawati, Endang and Ramdan, Ade and Pardede, Hilman Ferdinandus},
  journal={Jurnal Elektronika dan Telekomunikasi},
  volume={21},
  number={1},
  pages={19--26},
  year={2021}
}

@article{boll1979suppression,
  title={Suppression of acoustic noise in speech using spectral subtraction},
  author={Boll, Steven},
  journal={IEEE Transactions on acoustics, speech, and signal processing},
  volume={27},
  number={2},
  pages={113--120},
  year={1979},
  publisher={IEEE}
}

@article{van2009speech,
  title={Speech enhancement with multichannel Wiener filter techniques in multimicrophone binaural hearing aids},
  author={Van den Bogaert, Tim and Doclo, Simon and Wouters, Jan and Moonen, Marc},
  journal={The Journal of the Acoustical Society of America},
  volume={125},
  number={1},
  pages={360--371},
  year={2009},
  publisher={AIP Publishing}
}

@inproceedings{commonvoice:2020,
  author = {Ardila, R. and Branson, M. and Davis, K. and Henretty, M. and Kohler, M. and Meyer, J. and Morais, R. and Saunders, L. and Tyers, F. M. and Weber, G.},
  title = {Common Voice: A Massively-Multilingual Speech Corpus},
  booktitle = {Proceedings of the 12th Conference on Language Resources and Evaluation (LREC 2020)},
  pages = {4211--4215},
  year = 2020
}

@inproceedings{wang-etal-2021-voxpopuli,
    title = "{V}ox{P}opuli: A Large-Scale Multilingual Speech Corpus for Representation Learning, Semi-Supervised Learning and Interpretation",
    author = "Wang, Changhan  and
      Riviere, Morgane  and
      Lee, Ann  and
      Wu, Anne  and
      Talnikar, Chaitanya  and
      Haziza, Daniel  and
      Williamson, Mary  and
      Pino, Juan  and
      Dupoux, Emmanuel",
    booktitle = "Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.acl-long.80",
    pages = "993--1003",
}


@article{maccallum2011effects,
  title={Effects of low-pass filtering on acoustic analysis of voice},
  author={MacCallum, Julia K and Olszewski, Aleksandra E and Zhang, Yu and Jiang, Jack J},
  journal={Journal of Voice},
  volume={25},
  number={1},
  pages={15--20},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{pellegrino2018effect,
  title={The effect of ageing on speech rhythm: A study on Zurich German},
  author={Pellegrino, Elisa and He, Lei and Dellwo, Volker},
  year={2018},
  organization={ISCA}
}

@inproceedings{ramdinmawii2016gender,
  title={Gender identification from speech signal by examining the speech production characteristics},
  author={Ramdinmawii, Esther and Mittal, VK},
  booktitle={ICSC},
  pages={244--249},
  year={2016},
  organization={IEEE}
}



@article{lius,
  title={Accuracy and fairness trade-offs in machine learning: a stochastic multi-objective approach},
  author={Liu, S. and Vicente, L.N.},
  journal={Comput Manag Sci},
  volume={19},
  pages={513--537},
  year={2022},
  publisher={Springer}
}

@article{chen2006new,
  title={New insights into the noise reduction Wiener filter},
  author={Chen, Jingdong and Benesty, Jacob and Huang, Yiteng and Doclo, Simon},
  journal={IEEE Transactions on audio, speech, and language processing},
  volume={14},
  number={4},
  pages={1218--1234},
  year={2006},
  publisher={IEEE}
}

@inproceedings{osako2015complex,
  title={Complex recurrent neural networks for denoising speech signals},
  author={Osako, Keiichi and Singh, Rita and Raj, Bhiksha},
  booktitle={2015 IEEE workshop on applications of signal processing to audio and acoustics (WASPAA)},
  pages={1--5},
  year={2015},
  organization={IEEE}
}


\end{thebibliography}




